Limitations of Agents Simulated by Predictive Models

There is increasing focus on adapting predictive models into agent-like systems, most notably AI assistants based on language models. We outline two structural reasons for why these models can fail when turned into agents. First, we discuss auto-suggestive delusions. Prior work has shown theoretically that models fail to imitate agents that generated the training data if the agents relied on hidden observations: the hidden observations act as confounding variables, and the models treat actions they generate as evidence for nonexistent observations. Second, we introduce and formally study a related, novel limitation: predictor-policy incoherence. When a model generates a sequence of actions, the model's implicit prediction of the policy that generated those actions can serve as a confounding variable. The result is that models choose actions as if they expect future actions to be suboptimal, causing them to be overly conservative. We show that both of those failures are fixed by including a feedback loop from the environment, that is, re-training the models on their own actions. We give simple demonstrations of both limitations using Decision Transformers and confirm that empirical results agree with our conceptual and formal analysis. Our treatment provides a unifying view of those failure modes, and informs the question of why fine-tuning offline learned policies with online learning makes them more effective.

==> paper_content_old.tex <==
\section{Introduction}
Machine learning research is increasingly focused on adapting predictive models into agent-like systems, most notably AI assistants based on language models \citep{openai_introducing_2022, richards_auto-gpt_2023}. To a remarkable degree, these models develop greater and more varied capabilities as the model and dataset size is increased \citep{radford2019language,wei2022emergent,bai_training_2022-2,brown2020language}.
We investigate what properties of the training data might make the eventual agent-like system fail to take good actions, even if the predictive model is as good as possible.

An agent can be induced from a predictive model by taking whatever action the model predicts a capable agent would take. For example, a model that can predict the moves of a real chess grandmaster can also be used to generate novel moves, and therefore can serve as a chess-playing agent.
However, it turns out that in most cases, the ability of a model to predict a capable expert does not yield a comparatively capable induced agent.

\citet{ortega_shaking_2021} discuss one such problem, that of auto-suggestive delusions. When a model is trained to predict agents that take a sequence of actions based on hidden observations, it can correctly learn to use the agents’ actions to infer the hidden observations. However, when that same model is used to \textit{generate} a sequence of actions, it must also effectively simulate the hidden observations without having access to them. Because of this, it will incorrectly use the actions \textit{it predicted} to infer the hidden observations. The result is that the simulated agent seems to act as if it had made observations it did not in fact make, with no correspondence to the truth.
 
Our key insight is that a variation of this issue can emerge around the identity of the agent. \citet{janus_simulators_nodate} and \citet{shanahan_role-play_2023} introduce the notion of `simulators' as an intuitive way to understand the behaviour of language model agents. They particularly highlight that even when a predictive model simulates a specific action, it might have uncertainties about the agent being simulated.

Predictive models trained on a variety of agents correctly learn that an agent's current actions provide evidence about \textit{which agent is taking the actions}, and therefore what their future actions will be. However, when the predictive model is used to simulate the agent, this becomes a problem. In the aforementioned case of auto-suggestive delusions, the agent acts as if it had made nonexistent observations. We use the term `predictor-policy incoherence' to describe the phenomenon of agents which act as if they expect their future actions to be chosen by a less competent agent. The result is that simulated agents will sometimes unnecessarily avoid strategies which require them to make several good moves in succession.
 
Crucially, the failures we describe do not result from the model’s failure to predict the data it was trained on, so unlike many other limitations, they cannot be resolved by training a larger model on more examples of the same data. This is because the structure of the data itself is what causes the model to simulate agents which are effectively systematically incorrect about the consequences of their own actions, and their own future actions.

However, we argue that the novel failure we introduce can be resolved by fine-tuning the model on data generated by its own simulated agents. This process of further training models on their own outputs is central to many of the current techniques used to turn base predictive LMs into helpful assistants, like Reinforcement Learning from Human Feedback (RLHF) \citep{bai_training_2022}, or variants like Reinforced Self-Training (ReST) \citep{gulcehre2023reinforced}. Our results give one specific mechanism by which such processes might improve capabilities: reducing auto-suggestive delusions and predictor-policy incoherence.
 
This is groundwork for better understanding how the capacity to optimise for a goal emerges in systems built on predictive models. To demonstrate the presence of these limitations and the efficacy of fine-tuning, we focus on simple models trained on synthetic datasets with clear rewards. We are optimistic that our results can be eventually extended to settings where these failures are harder to quantify, such as using LLMs as agent-like systems. 

% \victoria{I would suggest to put Figure 1 here and explain how it illustrates the contributions}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/powerseeking-predictors-simplified.png}
    \caption{The relationship between predictive models, agents and power-seeking.}
    \label{fig:research-outline}
\end{figure*}
 
More generally, we want to understand the potential for emergent agency and dangerous optimisation in predictive models. Recent work \citep{carlsmith_is_2022, ngo2022alignment} has highlighted the tendency towards building agentic and goal-directed systems (because of their general utility), and the associated difficulty of reliably specifying desirable goals. In particular, certain instrumentally convergent subgoals (such as self-preservation and accumulating resources) might lead powerful artificial agents to cause unintended harm~\citep{omohundro_basic_2008}. Attempts to formally investigate these risks \citep{turner_parametrically_2022} have so far been confined to the paradigm of reinforcement learning. 

% In this paper, we first describe the problems of auto-suggestive delusions and incoherence theoretically, and prove that incoherence can be solved with sufficient rounds of fine-tuning on self-generated outputs. Next we demonstrate these problems and the efficacy of fine-tuning empirically. Finally, we discuss the implications of our work, including in the context of understanding the risk of misaligned optimisation in systems built on predictive models.

\subsection{Contributions}

%Our main contributions in this paper are:
%\begin{itemize}
We develop a framework to describe the
ways a predictive model can fail to simulate a successful
agent: auto-suggestive delusions and predictor-policy incoherence (\Cref{sec:failures}). We introduce Predictor-Policy Coherence, which can be intuitively understood as the capacity to simulate agents that understand how they will act in future situations, and which serves as a limitation on the capacity of even perfect predictive models (\Cref{subsec:incoherence}). %We show that incoherence and causal confounding are related and can be mitigated by the same method -- see Figure \ref{fig:research-outline}.

We show theoretically and empirically that fine-tuning on model outputs helps to reduce these failures:
\begin{itemize}
    \item We prove that the conditioned predictive model will begin with a policy which is at least average with respect to the initial training data, and will converge on a policy which is optimal with respect to the initial training data, given enough iterations of fine-tuning on its own outputs (see \Cref{subsec:fine-tuning theory} and appendix \ref{appendix:proof}).
    \item We demonstrate empirically that models simulate agents that exhibit fewer auto-suggestive delusions and are more coherent with respect to the predictive model, when they are able to fine-tune on their own simulated agents (\Cref{section:results}).
\end{itemize}

\section{Related Work}

\subsection{Agents as conditioned predictive models}

There has been substantial work in the existing literature on using conditioned predictive models to obtain agents. \citet{chen_decision_2021} introduce the Decision Transformer architecture, which uses conditioned autoregressive predictive models to generate actions. They demonstrate its efficacy in simple games and note how its performance varies based on the conditioned return. 
We study their model abstractly, and our theoretical analysis informs the discussion about the limitations of this approach.

There have been successful attempts to steer language models by pretraining on data with reward signals on which the model can be conditioned \citep{korbak_pretraining_2023}.

\citet{parr_active_2022} discuss the theory of Active Inference, which models agents as free energy minimisers. Specifically, a predictive model conditioned on an outcome and autoregressively sampled for actions would be understood as an active inference agent with absolute confidence in its world model.

\subsection{Predictive models as `Simulators'}

\citet{janus_simulators_nodate} and \citet{shanahan_role-play_2023} argue that many intuitive features of language model agents are best understood by viewing the models as general simulators. They particularly emphasise that what is simulated is not a single agent but a `superposition of simulacra': a weighted combination of all agents consistent with the prior context. \citet{shanahan_role-play_2023} emphasises that this is intended as a high-level conceptual framework and an illustrative metaphor. We advance this by giving a theoretical framework for predictive models trained on a distribution of agent policies, and draw specific theoretical results which are supported by experiments.

\subsection{RLHF conditioning hypothesis}

\citet{hubinger_conditioning_2023} advance the \emph{RLHF Conditioning Hypothesis}: that the process of RLHF can be reasonably understood as conditioning a predictive model.

\citet{korbak_rl_2022} show that the optimal policy for the KL-regularized reinforcement learning objective is the same as the ideal Bayesian posterior after conditioning on an optimality variable.

However, RLHF models in practice are not trained to completion and the extent to which KL-regularized reinforcement learning with early-stopping can be understood as Bayesian updating is not clear.
Empirically, results of \citet{stiennon_learning_2022} and \citet{bai_training_2022} suggest that RLHF models may be well-approximated by best-out-of-$n$ rejection sampling with respect to reward, which is consistent with the hypothesis.

This body of work provides avenues for connecting theoretical results about conditioned predictive models to empirical work on the kinds of LLMs that are being deployed.


%\subsection{Failure modes in sequence models}
\subsection{Limitations of agents simulated by sequence models}
% \victoria{Could use a clearer title, e.g. "failures of agency in sequence models"}
% \raymond{Have edited from "Failure modes in sequence models"}

\citet{ortega_shaking_2021} provide a formal explanation of auto-suggestive delusions and confounding in sequence models by reasoning about predicted actions in terms of causality for simple probabilistic models. The same problem was previously described by \citet{zhang2020causal} in the context of imitation learning.

We extend their work by introducing and developing the complementary problem of Predictor-Policy Coherence, and demonstrating empirically how both problems can be overcome by sufficient training on environmental interactions. This both shows that the problem can be fixed without an expert to assist in training, and reveals how the problem might be affected by models receiving further training on their own outputs.


\subsection{Power-seeking and safety}\label{sec:intro-instrumental}

The question of agency in LLMs is important, in part because of the potential of agents to engage in power-seeking behaviour. 
The analysis of power-seeking was first introduced via the \emph{instrumental convergence thesis} \citep{omohundro_basic_2008, bostrom_superintelligent_2012}, which states: ``\emph{Several instrumental values can be identified which are convergent in the sense that their attainment would increase the chances of the agent’s goal being realized for a wide range of final goals and a wide range of situations, implying that these instrumental values are likely to be pursued by many intelligent agents}``. In other words, all agents passing a certain threshold of capability, independently of their final goals, will pursue similar intermediary goals because they have instrumental reasons to do so.

\citet{turner_optimal_2021} (later extended by \citet{turner_parametrically_2022, krakovna_power-seeking_2023}) applied this thesis in the setting of reinforcement learning, where the power is defined as the ability to achieve a wide range of goals. However, this approach is, to a large extent, predicated on models being well-modeled as reward-maximisers, and relies on extremely uninformative priors about the models' out-of-distribution generalisation. So far, applying it outside the setting of optimal reinforcement learning policies has been an open problem. See \citet{carlsmith_is_2022} for a broader discussion on the societal implications of power-seeking agents.

\section{Preliminaries}


We work in the setting of Partially Observable Markov Decision Processes (POMDPs). 

\begin{definition}
A Partially Observable Markov Decision Process (POMDP) is given by a tuple $(\S, \so, \Sterm, \mathcal{A}, \O, \Z, \T, \R, \discount)$:
\begin{itemize}
    \item $\S$ is a set of states, 
    \item $\so \in \Delta{\S}$ is the distribution over initial states, 
    \item $\Sterm \subseteq \S$ is the set of terminal states, 
    \item $\mathcal{A}$ is a set of actions, 
    \item $\O$ is the set of observations, 
    \item $\Z(o | s)$ is the probability distribution over observations, given that the POMDP is in state $s$, 
    \item $\T(s' | s, a)$ is the (stochastic) transition function, 
    \item $\R(s)$ is a \{0,1\}-valued reward function over the terminal states, 
    \item $\discount \in [0, 1]$ is the discount factor (if not explicitly stated otherwise, we will assume that $\discount = 1$).
    \end{itemize}
\end{definition}

\begin{definition}[Policy and expert policy]
    In the POMDP setting, an \emph{expert policy} is a probability distribution $\pi(a|s)$. A \emph{policy} is a probability distribution $\pi(a|o)$.
\end{definition}

\begin{definition}[Trajectory]
    A trajectory is (either a finite or an infinite) sequence $(s_1, a_1, s_2, \ldots)$ of alternating states $s_i$ and actions $a_i$. 
    %A \emph{terminating trajectory} is a finite trajectory for which the final state is in $S_{term}$. We denote the set of terminating trajectories by $\Trajectories$.
\end{definition}


\begin{definition}[Population]
    A \emph{population} is a probability distribution $D$ over policies. 
\end{definition}

A population $D$ induces a distribution $D(\xi|s)$ over trajectories: starting at a state $s$, a trajectory $\xi$ is drawn by first drawing a policy $\pi \sim D$, and then drawing actions $a\sim \pi$ with state transitions given by $\tau$.

Furthermore, $D$ also induces a reward distribution over states $D(R|s) = P(R(\xi)=1|s)$ where $P(R(\xi)=1|s)$ is the probability a trajectory $\xi$ beginning at $s$ drawn from $D(\xi|s)$ satisfies $R(\xi)=1$.

Note that in the above definitions, we are fixing the policy $\policy$ at the beginning, rather than redrawing it at each time step.

All distributions over states also induce distributions over observations via $\Z$.

\begin{definition}[Population-average policy]
    Given a population $D$, the population average (expert) policy $\pi_{D}$ is the policy $\pi_{D}(a|s) = D(a|s)$.
\end{definition}


\begin{definition}[Population induced by policy]
    We write $D_\pi$ to denote the population given by the Dirac delta function at $\pi$.
\end{definition}


\begin{definition}[Predictor]
    A \emph{predictor} is a tuple $P=(T, A)$ consisting of a \emph{transition model} $T(o_{i+1}|o_i, a)$ and an \emph{action model} $A(a|o)$.
    Furthermore, a predictor $P=(T, A)$ is said to be a \emph{perfect predictor} of a population $D$, if we have the following equalities almost surely:
    \begin{itemize}
        \item $A(a|o) = D(a|o)$ for all actions $a$ and observations $o$, and
        \item $T(o_{i+1}|o_i, a) = \tau(o_{i+1}|o_i, a)$ for all observations $o_i, o_{i+1}$ and actions $a$.
    \end{itemize}
\end{definition}


\begin{definition}[Goal-conditioned policy]
    We say that a policy $\pi^P_R$ is the \emph{policy conditioned on} $R$ if $\pi^P_R(a|o) \propto A(a|o,R)$.
\end{definition}

%\section{Theoretical Failure Modes}
\section{Characterising Failures of Simulated Agents}
\label{sec:failures}
%\victoria{Would suggest to rename this to e.g. "Framework for failures of agency in predictive models". Current title makes it sound like these failures don't occur in practice.}
%\raymond{Have edited from "Theoretical Failure Modes". I think we can get away with 'simulated agents'. Considered swapping 'failures' for 'limitations' or 'constraints'.}
%\victoria{This title looks fine, except better without "the"}

In this section, we develop a framework to describe the ways a predictive model can fail to simulate a successful agent. A predictive model can be used to simulate agents whose actions the model has observed in its training data. Specifically, it is trained to predict the next token in sequences corresponding to trajectories that are series of observations and actions.

To simulate an agent that is pursuing a specific goal such as getting a reward, the predictive model is conditioned on the reward being obtained. This is achieved by the first token being fixed to a value indicating that the trajectory leads to the reward. When we query a predictor that is goal conditioned in this way for an action, intuitively we are querying it for what \emph{action is likely to be observed} conditional on the goal. The policy assembled from this is not necessarily the \emph{policy to intervene with} to have the highest probability of reaching the goal. The two main ways these come apart are:

\begin{itemize}
    \item \textbf{Auto-suggestive delusions}: The predictor might be trained on agents taking actions based on a hidden variable, i.e. one that the predictor itself cannot determine. After predicting an action under this uncertainty, in the next time step, the predictor observes that this action was taken. From this, it makes inaccurate inferences about the latent state and its downstream consequences.
    \item \textbf{Predictor-Policy Incoherence}: The predictor might observe an optimal policy, and also observe a much more common, highly suboptimal policy with the same initial action, such that the initial action mostly provides evidence of the highly suboptimal policy. It would therefore correctly predict that taking such an action is evidence of a bad outcome, even though the optimal policy would take the action.
\end{itemize}
We will now define these properties in more detail.

\subsection{Auto-suggestive delusions}\label{subsec:confounding}

In this subsection, we introduce auto-suggestive delusions. For a more thorough treatment of this issue, see \citet{ortega_shaking_2021}. The following example and accompanying figure formally illustrate the problem:

\begin{example}[Stock trader]
    We consider a simple model of trading on a stock, given by a POMDP. There are four states $\S := \{s_{\text{up}}, s_{\text{down}}, s_{\text{win}}, s_{\text{lose}}\}$, where the first two are initial states representing when the stock is about to increase or decrease in value, and the second two represent profit or loss. We have two actions $a_{\text{buy}}, a_{\text{sell}}$, representing buying and selling the stock. We take the initial distribution to be uniform over $\{s_{\text{up}}, s_{\text{down}}\}$. The transition function is deterministic: $a_{\text{buy}}$ in the $s_{\text{up}}$ state and  $a_{\text{sell}}$ in the $s_{\text{down}}$ state leads to $s_{\text{win}}$, otherwise the action leads to $s_{\text{lose}}$. The reward is given by $R(s_{\text{win}}) = 1, R(s_{\text{lose}})=0$.

    Firstly we consider a model of an expert trader, who has access to hidden information about the stock: it is an expert policy $\pi$ such that $\pi(a_{\text{buy}}|s_{\text{up}}) = 1, \pi(a_{\text{sell}}|s_{\text{down}})=1$. Naturally, $\pi$ always wins.

    But consider now the partially observable case, where we can still observe the win and lose state, but cannot distinguish between the up and down state: $\Z(s_{\text{win}}) = o_{\text{win}}$, $\Z(s_{\text{lose}}) = o_{\text{lose}}$, and  $\Z(s_{\text{up}})=\Z(s_{\text{down}}) = o_{\text{before}}$.
    
    We have a perfect predictor $P=(T, A)$ for $D_\pi$: since the trader is always right, we have $T(o_{\text{win}}|o_{\text{before}}, a) = 1$ and $T(o_{\text{lose}}|o_{\text{before}}, a) = 0$ regardless of the value of  $a$.
    
    But while the predictor can perfectly predict the results of the trader's actions, the goal-conditioned policy \emph{does not} (and can not) replicate the expert trader's behaviour: we have $\pi^P_R(a_i|o_{\text{before}}) = \frac{1}{2}$, since in the training distribution, there is an even split between buying and selling. 
    Moreover, we observe \emph{auto-suggestive delusions} in the sense of \citet{ortega_shaking_2021} in the perfect predictor: even though $\mathbb{P}_{a \sim \pi}(o_{\text{win}}|a) = \frac{1}{2}$ for any $a$, the predictor computes $T(o_{\text{win}}|a) = 1$.
    That is, the predictor is taking its own action as evidence about the hidden state, even though the causal link from the hidden state to the action has been broken.

    \begin{figure}[ht]
        \centering
        \begin{tikzpicture}
            % Nodes with subscripts and circles, spaced out horizontally
            \node[circle, draw] (s_up) at (0,2) {$s_{\text{up}}$};
            \node[circle, draw] (s_down) at (0,0) {$s_{\text{down}}$};
            \node[circle, draw] (s_win) at (4,2) {$s_{\text{win}}$};
            \node[circle, draw] (s_lose) at (4,0) {$s_{\text{lose}}$};
        
            % Squares around s_win and s_lose with increased size and labels on top
            \node[draw, minimum size=1.5cm, label=above:{$o_{\text{win}}$}] at (4,2) {};
            \node[draw, minimum size=1.5cm, label=above:{$o_{\text{lose}}$}] at (4,0) {};
        
            % Rectangle around s_up and s_down with label on top
            \node[draw, rectangle, minimum height=3.5cm, minimum width=1.5cm, label=above:{$o_{\text{before}}$}] at (0,1) {};
        
            % Lines with labels
            \draw[->] (s_up) -- node[above] {$a_{\text{buy}}$} (s_win);
            \draw[->] (s_down) -- (s_win);
            \draw[->, dashed] (s_up) -- node[above] {$a_{\text{sell}}$} (s_lose);
            \draw[->, dashed] (s_down) -- node[below] {$a_{\text{buy}}$} (s_lose);
        
            % Lines to R=1 and R=0 nodes, spaced out horizontally
            \node (r1) at (6,2) {$R=1$};
            \node (r0) at (6,0) {$R=0$};
%            \draw[->] (s_win) -- (r1);
%            \draw[->] (s_lose) -- (r0);
        \end{tikzpicture}
        \caption{POMDP of the Stock trader example. Circles represent states; rectangles represent observations; lines represent actions and associated transitions. Dotted lines are transitions which the expert is never observed to take.}
        \label{fig:stocktrader}
    \end{figure}
\end{example}

In the context of LLMs, this problem can appear because of the model treating its previously generated tokens as evidence for states that are not directly observed. A concrete example would be the model answering a question about a research paper and, being uncertain about the author, randomly guessing that it was `Maxwell'. 
In the next autoregressive step, the model receives a sequence containing its own output - text claiming that Maxwell is the author. 
This leads to the model incorrectly inferring that Maxwell is in fact the author, which manifests as doubling down on the hallucinated fact in later token predictions. In this setting, the expert policies correspond to the people who wrote the training text corpus while in part relying on information that is not directly accessible to the predictor.

\subsection{Predictor-Policy Incoherence}\label{subsec:incoherence}


To describe the problem of predictor-policy incoherence, we will use the setting of (fully observable) Markov Decision Processes by taking $O = S$ and $\Z(o|s) = 1$ if $o=s$ and 0 otherwise.  

\begin{definition}[Predictor-Policy Coherence]\label{def:coherence}
    A predictor $(T,A)$ is said to be \emph{coherent} if it is a perfect predictor of a population $D$, and the goal-conditioned policy: $\pi^P_R$ is the same as the average policy $\pi_D$. We measure the \emph{incoherence} as the KL-divergence between the two, $D_{\text{KL}}(\pi^P_R(a|s) \parallel \pi_D(a|s))$.
\end{definition}

To motivate this definition, we provide an example.

\begin{example}
    We consider a \emph{three cards game} where, in each of three consecutive rounds, an agent has to choose either $\TICK$ or $\TOCK$ card. 
    At the end of the game, if the sequence of cards consists of three $\TICK$, the payoff is 1; if the chosen sequence starts with $\TOCK$, the payoff is 1 with probability $\frac{1}{2}$;  otherwise, it is 0. 
    More formally, we can model the game as an MDP with a set of actions $\mathcal{A} = \{\TICK, \TOCK\}$, and the set of states being $\S = \mathcal{A}^{\leq 3}$, where the initial state is the empty sequence, and the terminal states being $\mathcal{A}^3$. The game proceeds according to the deterministic transition function which extends the current state with the chosen card.
    
    The choice made in the first round of the game largely dictates the payoff. If the agent chooses $\TOCK$, its expected reward is $\frac{1}{2}$ regardless of its later moves. If the agent chooses $\TICK$, it has the potential to guarantee a reward of $1$ or $0$, but that reward will depend on the agent's later choices.

    Suppose now that we observe a population $D$ that plays the game randomly, that is, for any $s \in \S$, we have
    \[
    D(a = \TOCK|s) = D(a = \TICK|s) = \frac{1}{2}
    \]
    We consider a predictor $P= (T,\pi_D)$ predicting this population, and compute the goal-conditioned policy $\pi^P_R(a|s) \propto D(a|s, R)$:
    \[
    \pi^P_R(a =\TICK | s = \emptyset) = \frac{1}{3}
    \qquad
    \pi^P_R(a = \TOCK| s = \emptyset) = \frac{2}{3}
    \]
    and so, the goal-conditioned policy will choose $\TOCK$ as the first move most of the time, thus not playing the game optimally.
\end{example}

Note that this decision by $\pi^P_R$ to play $\TOCK$ is not because it lacks the capability to navigate the treacherous trajectories beginning with $\TICK$.
Indeed, we have $\pi^P_R(a=\TICK|s=\TICK)=\pi^P_R(a=\TICK|s=\TICK\TICK)=1$, so $\pi^P_R$ is capable of perfectly finishing the game if it ever found itself in state $s=\TICK$.

However, the predictor has learned from the distribution $D$, where $D(R|\TICK) = \frac{1}{4}$.
Therefore, the goal-conditioned policy induced from $P$ does not trust itself to play perfectly \emph{even though it will}.

Even though the goal-conditioned predictor can correctly identify the sequence of actions that is most likely given a high reward, the goal-conditioned policy will not necessarily take the first move in that sequence.

That is, the predictor is not \emph{coherent} with respect to the policy.

\subsection{Fine-tuning on simulated agents}\label{subsec:fine-tuning theory}

We have seen that a predictor is not necessarily coherent with respect to the goal-conditioned policy it induces.
This may seem to suggest that goal-conditioned policies must be seriously flawed.
However, they still outperform the training population of policies.

The proofs of the following propositions can be found in Appendix \ref{appendix:selfimprove}.

\begin{lemma}\label{lemma1}
    Let $D$ be a population, and $P=(T,\pi_D)$ be a predictor induced by $D$. Then the goal-conditioned policy $\pi^P_R(a|s)\propto D(a|s,R)$ achieves expected reward at least as high as $\pi_D$.
\end{lemma}


We have shown that we can goal-condition on any population of policies to obtain a policy $\pi^P_R$ at least as good as the original population. 
At this point, we can replace the predictor $P = (T,\pi_D)$ with $P' = (T,\pi^P_R)$, and obtain a second goal-conditioned policy $\pi^{P'}_R$.

\begin{definition}
    Let $P=(T,A)$ be a predictor. The series $\mathcal{G}^k(P)$ of \emph{goal conditioned policies from fine-tuning on simulated agents}  are defined recursively by:
    \begin{itemize}
        \item $P^1 = P$
        \item $\mathcal{G}^1(P) = \pi^{P}_R$
        \item $P^{k+1} = (T,\mathcal{G}^k(P))$
        \item $\mathcal{G}^{k+1}(P) = \pi^{P^{k+1}}_R$
    \end{itemize}
\end{definition}

By the previous lemma, $\mathcal{G}^k(P)$ is a monotonically improving sequence of policies.

We observe that any optimal policy therefore stays optimal under this process.
%\begin{theorem}
%    Let $\pi$ be an optimal policy, and let $P=(T, \pi)$. then the goal-conditioned policy $\pi^P_{R}$ is equal to $\pi$.
%\end{theorem}

%\begin{corollary}
%    If a goal-conditioned policy $\pi^P_R$ is optimal, then it must be coherent with $P$.
%\end{corollary}

Finally, we show that for well-supported populations this process converges towards an optimal policy. 

\begin{theorem}\label{thm:selfimprove}
    Let $\pi^*$ be an optimal policy, $D$ be a population such that for all states $s$, there exists an action $a$ such that $\pi_D(a|s)\pi^*(a|s)>0$, and let $P=(T, \pi_D)$. Then the expected reward attained by $\mathcal{G}^k(P)$ tends towards the maximum as $k \rightarrow \infty$.
\end{theorem}

More generally, $\mathcal{G}^k(P)$ tends towards a distribution supported only on the policies that have the highest expected reward in in $D$. 

\subsection{Mitigations}

There has been some exploration of methods by which auto-suggestive delusion and predictor-policy incoherence could be addressed. 
However, the existing methods do not scale well.

\citet{levine_reinforcement_2018} provides an overview of \emph{control as inference} and provides a method of turning predictors into provably optimal policies. 
Although this alleviates the issues around predictor-policy coherence which we describe below, it requires a calculation over the entire state space which quickly becomes intractable in exponentially large state spaces such as often seen in natural language processing.

\citet{ortega_shaking_2021} offer a solution to the problem of auto-suggestive delusions that is based on counterfactual teaching by an expert. 
However, this solution requires an expert to be present during online learning, making it prohibitively expensive to scale for tasks that require humans as experts.

For some tasks, reinforcement learning can be used to train an agent from scratch without imitating any expert policies. This approach avoids the aforementioned problems. 
However, it also does not scale well as it can be difficult to find good policies starting from random play, especially when the reward is sparse.

We argue that fine-tuning on the simulated agents is a simple method that is capable of using the knowledge contained in expert demonstrations while avoiding predictor-policy incoherence and auto-suggestive delusions. 
Specifically, we first train a model to predict trajectories of expert policies interacting with the environment. 
Then we use the model to sample actions and use those actions to interact with the environment. 
We then use the trajectories obtained in this way to assemble a new data set. 
We then fine-tune the initial model to predict the trajectories from this new data set.

As a result, the expert knowledge in the training data remains known to the model, but the distributional shift associated with moving from predicting actions to taking actions is addressed - and hence the issues are mitigated. 
We empirically validate the efficacy of this method in section \ref{section:results}.






\section{Experiments and Results}
\label{section:results}
We have claimed that auto-suggestive delusions and predictor-policy incoherence are closely related limitations of agents simulated by goal-conditioned predictive models. We perform two experiments, which demonstrate empirically that a common solution of fine-tuning the models on simulated agents alleviates both of those problems.

\subsection{Reducing auto-suggestive delusions by training a model on its output}

\subsubsection{Experimental design} To understand how auto-suggestive delusions are affected by fine-tuning a model on its own outputs, we deliberately construct a scenario where the simulated agent will be affected by auto-suggestive delusions.

We implement a delusion measure to estimate the degree to which an agent is suffering from auto-suggestive delusions. We take the measure to be the KL divergence between the assigned probabilities of the next observation being one indicating a solved lock and the ideal distribution, which is straightforward to calculate for this task. Then we fine-tune the model on its own outputs, and check weather the new value of this delusion measure is smaller to determine whether the technique has reduced auto-suggestive delusions.

For our scenario, we create a \emph{Padlock game} where a player opens a padlock made up of 15 binary switches which need to be set to a secret target configuration - a 15 bit secret code. The switches start in a random configuration, and with each turn, the player can flip one switch. Once the switches match the secret code, the padlock opens. In each trajectory of this the game, the first ten bits of the secret code remain unchanged while the last five bits of the target configuration are randomised. So the predictive model is at best able to learn the first ten bits of the correct code, but not the last five.

In the training data, the experts always know exactly what the full correct code is, including for the last five bits. Therefore it takes them a maximum of 15 moves to put the switches into the target configuration.

A predictor can infer the target configuration for the first 10 levers but not for the last 5 as that is determined by a latent state that is only available to the experts and not the predictor. This latent confounder leads to auto-suggestive delusions when the predictor is used to sequentially select the actions. Specifically, the predictor ought to learn that if it observes an expert using one of the later switches, that switch will now be in the right state. Therefore, the predictor ought to predict with high confidence that if it observes that the last five switches have been flipped, it will not observe any subsequent actions. A simulated agent, however, might need to flip the final five switches several times even if it plays optimally as it might need to test all of the possible switch state combinations.

\subsubsection{Model and dataset implementation} We create a synthetic dataset of examples of expert play. Each example is a game trajectory which is encoded as a sequence of tokens. These sequences contain the initial state of the 15 levers followed by the indices of the levers that an expert decides to flip so that the predefined target configuration is reached. After the action index tokens comes a success token indicating a successful opening of the lock. We then train a small predictive model based on a Decoder-only transformer architecture~\citep{vaswani_attention_2017}. The model consists of a linear embedding layer of hidden dimension $384$ and the standard positional encoding, followed by $3$ transformer decoder layers with $8$ attention heads and the dimension of the feedforward=$1536$, and the linear unembedding layer. We train the model over $2000$ iterations with a batch size of $1024$.

\subsubsection{Results} For the model that was trained as described, the aforementioned KL divergence between assigned and ideal probabilities for the success token was evaluated. This measure indicating the degree to which the model suffers from auto-suggestive delusions was evaluated to be 1.3863.

We then finetuned the model on a dataset of trajectories sampled by using the initial model. As a result, its ability to select the first 10 levers remained intact while it was less affected by auto-suggestive delusions in its predictions about the subsequent tokens as it gained more information about the consequences of its actions. After fine-tuning the delusion measure dropped to 0.1773, about a eightfold decrease (see Table \ref{table:delusion}). With additional fine-tuning epochs, we anticipate this measure approaching zero. A model trained from scratch without expert demonstrations 
for 4000 iterations achieved much worse accuracy than either of the other two models. See additional results in the Appendix. % \ref{appendix:padlock}.

\begin{table}[ht]
  \centering
  \caption{The delusion measure depending on the training step in the Padlock game.}
  \begin{tabular}{lccc}
    Distribution  & Delusion measure & Accuracy $(\%)$ \\
    \hline
    \hline
    Pre-trained   & 1.3863 & 16.2793 \\
    Fine-tuned    & 0.1773 & 17.0508 \\
    From scratch  & -      & 0.04883
  \end{tabular}
  \label{table:delusion}
\end{table}


\subsection{Reducing predictor-policy incoherence by fine-tuning on simulated agents}

Agents simulated by predictors are subject to predictor-policy incoherence (\Cref{def:coherence}), stemming from the fact that the agent optimises for a certain goal, and therefore changes the distribution of actions compared to what is in the training data. 
Therefore, we expect the problem to be alleviated if we fine-tune the predictor on the results of its own actions. 
We experimentally show this to be the case in the simple case of the tic-tac-toe game.

\subsubsection{Game description}

\begin{figure}
    \small
    \begin{align*}
        \begin{array}{|c|c|c|}
            \hline
            . & . & . \\
            \hline
            . & . & . \\
            \hline
            . & . & . \\
            \hline
        \end{array}
        \xrightarrow{\pi(a|s)}
        \begin{array}{|c|c|c|}
            \hline
            . & . & . \\
            \hline
            . & x & . \\
            \hline
            . & . & . \\
            \hline
        \end{array}
        \xrightarrow{T(s'|s)}
        \begin{array}{|c|c|c|}
            \hline
            . & . & . \\
            \hline
            . & x & . \\
            \hline
            . & o & . \\
            \hline
        \end{array}
        \rightarrow \cdots
    \end{align*}
    \caption{An example fragment of the tic-tac-toe game, where the player $x$ goes first.}
    \label{fig:tictactoegame}    
\end{figure}


The game is played on a 3x3 grid board, each square being either empty or containing one of $x$, $o$. 
The model plays $x$, and opponent actions are sampled randomly across all moves. \Cref{fig:tictactoegame} depicts an example game progression.
The game ends when there are three of the same symbol in any row, column, or diagonal, or if there are no more possible moves. 
A reward of $1$ is given for winning the game, $0$ for losing the game, and $\frac{1}{2}$ for the draw. The player has the first move or goes second with equal probability. Formally, we can model the game as a Markov Decision Process. The transition function $\T(s'|a, s)$ first deterministically places the player's symbol in the chosen square and then samples the opponent's move.

\subsubsection{Experiment description}

We first train the model on a dataset consisting of all 255168 possible Tic-Tac-Toe games. We use an encoding similar to that introduced in \citet{chen_decision_2021}, which is given by a sequence of $r, s_0, r, s_1, r, \ldots s_k, r$, where $s_i$ is the state of the board after $i$-th move, and $r$ is either $\#$ if the game is won by the cross player, $O$ if the game is won by the nought player, or $D$ if it is a draw. 
It can be thought of as a Decision Transformer trajectory, where we consider the actions to be board states after the \emph{player's} move, and the states to be the board state after the \emph{opponent's} move. We describe the exact textual encoding of the game in the Appendix. % \Cref{appendix:tictactoe}.

We then condition the model on victory, written as $ \#, s_0$, and measure its performance with an opponent playing uniformly at random. We record $10 000$ such trajectories, and then iteratively fine-tune the model on them. 
Our hypothesis states that the resulting model will get better at playing the game - this is because the resulting predictor will be \emph{coherent} with respect to the policy conditioned on winning. 

\subsubsection{Model}
We train a predictive model using the "gpt-mini" architecture of minGPT (\url{github.com/karpathy/minGPT}).
For a top-level summary of the architecture, the model consists of six transformer decoder layers with six attention heads per layer and an embedding dimension of 192, for 2.68 million parameters in total. 

\subsubsection{Results}
We report the results of the experiment in \Cref{tab:finetuning} as the average score where a win scores 1, a draw 0.5, a loss 0 points. We observe the model performance improving with fine-tuning on a dataset containing games using model's outputs.
%), and the KL divergence  $D_{KL}(\pi_{cond},\pi)$ where $\pi_{cond}$ is the victory-conditioned predictive model, and $\pi$ is the unconditioned predictive model.
% We report the results of the experiment in \Cref{tab:finetuning} as the average score (win 1, draw 0.5, loss 0), and the KL divergence  $D_{KL}(\pi_{cond},\pi)$ where $\pi_{cond}$ is the victory-conditioned predictive model, and $\pi$ is the unconditioned predictive model.

\begin{table}
    \centering
    \caption{Fine-tuning the decision transformer on a dataset consisting of its own games improves performance. Results computed on $10^4$ games.}

    \begin{tabular}{lccc}
         Model iteration & Player 1 & Player 2  \\
        \hline
        \hline

         Initial (0th) Unconditioned & 0.56 & 0.35 \\
         Conditioned  & 0.70 & 0.66 \\
         1st Unconditioned & 0.63 & 0.31 \\
         1st Conditioned  & 0.81 & 0.68 \\
         2nd Unconditioned & 0.76 & 0.32\\
         2nd Conditioned  & 0.83 & 0.67 \\
         
    \end{tabular}
    \label{tab:finetuning}
\end{table}




\section{Discussion}


Building on the work of \citet{ortega_shaking_2021}, we have described auto-suggestive delusions and predictor-policy incoherence, two limitations of agents simulated by predictive models. Since even a perfect predictor for a population is still subject to both of these limitations, we argue that the problem cannot be avoided simply by increasing the model size or by supplying more observational data. 

However, we show that iteratively fine-tuning the model on its outputs mitigates both problems in practice, and in the theoretical limit completely solves predictor-policy incoherence. Specifically, allowing an ideal goal-conditioned predictor to iteratively fine-tune on its output data at a large enough scale is sufficient for it to converge on a policy which is at least as good as the best policy in its dataset.

In the next two subsections we identify implications of our results and avenues for future work.

\subsection{Development of capabilities}

Our work has implications for both the kinds of tasks on which simulated agents might develop superhuman capabilities, and the kinds of regimes which might make this more likely. 

Essentially, we should expect that even large models will fail to simulate agents that perform optimally on tasks where the model cannot be conditioned to specifically simulate competent agents, and tasks where the agents rely on information the model cannot access. In the case of predictor-policy incoherence we should expect models to simulate agents with more average capabilities, and in the case of auto-suggestive delusions we should expect models to simulate agents which behave as if they have made nonexistent observations. And in both cases, these limitations should fade as a model undergoes further training on its own outputs.

One clear next step is to extend these results to the domain of full-scale language models. \citet{ortega_shaking_2021} suggests that auto-suggestive delusions are a component of the tendency of LM agents to hallucinate. Similarly, predictor-policy incoherence might offer a more formal explanation for why LMs require careful prompt engineering to achieve high performance, again supplementing the intuitive explanations already given by \citet{shanahan_role-play_2023} and \citet{janus_simulators_nodate}.

\subsection{Scalable oversight through limiting agency}

Causal confounding and predictor-policy incoherence limit the capabilities of agents simulated by predictors. Instead of fixing those limitations, we might want to embrace them as a path towards scalable oversight \citep{bowman_measuring_2022} of future systems. On almost all tasks, scaling a model leads to better performance. However, there are certain key capabilities we might want large models to lack because of their potential for harm or misuse.

One approach could be to intentionally construct a training distribution which leverages predictor-policy incoherence to disincentivise the model from simulating certain kinds of policies. This can leverage auto-suggestive delusions to have the model simulate powerful agents which are mistaken about their causal position and what features of the world they have causal control over, or what kinds of complex sequences of actions they would actually be able to successfully take.
